UStore: A Distributed Storage With Rich Semantics

Today's storage systems expose abstractions which are either too low-level (e.g., key-value store, raw-block store) that they require developers to re-invent the wheels, or too high-level (e.g., relational databases, Git) that they lack generality to support many classes of applications. In this work, we propose and implement a general distributed data storage system, called UStore, which has rich semantics. UStore delivers three key properties, namely immutability, sharing and security, which unify and add values to many classes of today's applications, and which also open the door for new applications. By keeping the core properties within the storage, UStore helps reduce application development efforts while offering high performance at hand. The storage embraces current hardware trends as key enablers. It is built around a data-structure similar to that of Git, a popular source code versioning system, but it also synthesizes many designs from distributed systems and databases. Our current implementation of UStore has better performance than general in-memory key-value storage systems, especially for version scan operations. We port and evaluate four applications on top of UStore: a Git-like application, a collaborative data science application, a transaction management application, and a blockchain application. We demonstrate that UStore enables faster development and the UStore-backed applications can have better performance than the existing implementations.

==> application_MVCC.tex <==
\subsection{MVCC based transaction processing}

\begin{figure}
\includegraphics[width=0.45\textwidth]{MVCC.pdf}
\caption{MVCC Architecture Components}
\label{fig:MVCC}
\end{figure}

For distributed transaction processing on top of U-Store, we discuss how a multiversion concurrency control protocol can be implemented by exploiting the the rich semantics and flexibility provided by U-Store. 
Our goal is to achieve the strengths of RDBMSs (i.e., SQL and ACID), and in the meantime to exploit the scalability and efficiency provided by U-Store. Our architecture is designed based on two principles.

The first principle is that it is a straightforward idea to leverage multiversion storage provided by U-Store to implement a MVCC based transactional processing architecture. 

The second principle that exploits flexibility and scalability, is to decouple transaction processing from data storage. Since
UStore provides a global data view, the data sharding and replications become transparent for transaction processing.
While in traditional RDBMS systems the transaction processing and data storage are tightly coupled, we can logically
separate these two components into two autonomous layers in UStore. This design makes flexibility and elasticity
possible as both two layers can be scaled out independently with regard to different workload demands.

Although UStore is a key-value storage, at the application view, the relational storage model is easier to use and maintain for database users.
To this end, we introduce the schema mapping between the table view and the key-value store. 
We assume the table view is row-based.
We combine the table name and the primary key of the table to be the keys of data as represented in UStore. 
Data of the same key may have multiple versions, and the versions are the same for both the storage and the application.
The value related to each key is the corresponding tuple. 
Since the data schema is defined by the application, after each tuple is retrieved, each field of the tuple can be accessed based on the schema.
Regardless of the data version, the above schema mapping is obviously valid because the combination of table name and primary key of the table must be unique in the flatten naming space.
On the other hand, data versions are directly mapped from the storage to the application.

\subsubsection{Snapshot Isolation}

In MVCC transaction processing, storage stores multiple versions of each data record. 
Whenever a record is updated, a new version of the record is created. 
During transaction processing, it is only allowed to access the records which has the versions written by already finished transactions and is never able to read the records written
by transactions that are running simultaneously. 
This protocol is called \textit{snapshot isolation} (SI)~\cite{berenson1995critique}, that guarantees
the ACID properties.

In SI, transactions perform operations on their own snapshot isolated from other transactions and finally check for conflicts
when tires to commit. The commit of a transaction \(T_{1}\) is only successful if none of the records in the write set has been
updated by another external transaction \(T_{2}\) that is commiting or has committed after \(T_{1}\) has started. If \(T_{1}\)
and \(T_{2}\) run parallelly and try to update the same record, two scenarios may happen. First, \(T_{1}\) reads a record before
it has been modified by \(T_2\), but later on, \(T_2\) will commit its modification and generate a new version of that record. In
this case, when \(T_1\) tries to commit its modification, it will notice that and aborts. Second, \(T_2\) has committed a write
to a record before \(T_1\) reads it. In this situation, \(T_1\) needs to notice the conflicts when it reads that record. 

\label{label:mvcc:architecture}
\subsubsection{System Architecture}

To provide SI across the transactions, each transaction needs to interact with a coordinator and a global
active version table. Figure~\ref{fig:MVCC} shows architecture components of the MVCC transactional processing.

{\bf Coordinator.} 
The coordinator provides a globally unique transaction ID for each transaction and maintains snapshot information by keeping tracks of all running transaction ID. 
From the snapshot information provided by the coordinator, one transaction is able to know all the transactions which happened before it, so it is allowed to read all the version of records written by those transactions.

We define the APIs for communication with the coordinator as follows: 

\begin{itemize}
\item $startTxn() \rightarrow (tid, ssDesp)$ \\
By calling this function at the start of the transaction, an unique transaction ID ($tid$) and a snapshot descriptor ($ssDesp$) are returned. 
These information are essential for the transaction to know the context of snapshot for execution.

\item $setCommitted(tid) \rightarrow void$ \\
Inform the coordinator about the successful commit of transaction.

\item $setAborted(tid) \rightarrow void$ \\
Inform the coordinator about the abort of transaction.
\end{itemize}

{\bf Active Version Table.} 
The active version table keeps track of the latest version for all the records. When a transaction tries to commit, it needs to make sure all its writes are working on the active (latest) version, otherwise, the transaction works on some stale records that means it needs to abort. 
Therefore, when a transaction is about to commit, it has to lock on all the data of its write set and materialize the updates of data in an atomic manner. 

To fulfill the above requirement, we define the schema of the active version table ($AV$) as follows: 
\[
AV(key, tid, version, latch)
\]
Recall that $key$ is the combination of table name and primary key of the table. 
$tid$ is the ID of transaction that performs the latest write on the data.
The coordinator guarantees that $tid$ is unique for each transaction.
$version$ is the latest version of data, which is necessary for the storage to retrieve the data with the specified version.
$latch$ is a lock without pending queue. 
It is used to provide the atomic semantic for transaction commit by updating $AV$.

Further, we define the APIs for interacting with the active version table as follows: 
\begin{itemize}
\item $getLatestVersion(key) \rightarrow (version, tid)$ \\
Retrieve the latest committed version of a data record and the ID of transaction which commits it.

\item $setLatestVersion(key, version, tid) \rightarrow void$ \\
Set the latest committed version of a record and the ID of transaction which commits it.

\item $acquireVersionLock(key, tid) \rightarrow true/false$ \\
When a transaction tries to commit, it requires to acquire the lock on the value of latest version for the records which it tries to update. 

\item $releaseVersionLock(key, tid) \rightarrow void$ \\
Release the lock on the value of latest version of a record.
\end{itemize}

\begin{algorithm}[t]
\AlgoFontSize
\DontPrintSemicolon

\SetKwFunction{funcBegin}{Begin}
\SetKwFunction{funcRead}{Read}
\SetKwFunction{funcWrite}{Write}
\SetKwFunction{funcCommit}{Commit}
\SetKwFunction{funcAbort}{Abort}
\SetKwFunction{funcGet}{Get}
\SetKwFunction{funcPut}{Put}
\SetKwFunction{funcMerge}{Merge}

\Func{\funcBegin{}}{
  $(tid,\ ssDesp) \gets startTxn()$\;
}

\BlankLine

\Func{\funcRead{key}}{
  $(latestVer,\ commitTid) \gets getLatestVersion(key)$\;
  \uIf{$commitTid \not\in ssDesp$}{
    \funcAbort{}\;
  }
  \Else{
    \funcGet{$key$, $latestVer$}\;
  }
}

\BlankLine

\Func{\funcWrite{$key$, $value$}}{
  \uIf{$key \in writeSet$}{
    $latestVer \gets writeSet(key)$\;
  }
  \Else{
    $(latestVer,\ commitTid) \gets getLatestVersion(key)$\;
    \lIf{$commitTid \not\in ssDesp$}{\funcAbort{}}
  }
  
  $writeSet(key) \gets \funcPut{key, latestVer, value}$\;
}

\BlankLine

\Func{\funcCommit{}}{
  \ForEach{$key \in writeSet$}{
    \If{$acquireVersionLock(key, tid) \textnormal{ is } false$}{
      \ForEach{$key \in writeSet$}{
        $releaseVersionLock(key, tid)$\;
      }
      
      \funcAbort{}\;
    }
  }
  
  \ForEach{$key \in writeSet$}{
    $(latestVer,\ commitTid) \gets getLatestVersion(key)$\;
    \If{$commitTid \not\in ssDesp$}{
      \ForEach{$key \in writeSet$}{
        $releaseVersionLock(key, tid)$\;
      }
      
      \funcAbort{}\;
    }
    
    \funcMerge{$key$, $latestVer$, $writeSet(key)$}\;
  }

  \ForEach{$key \in writeSet$}{
    $releaseVersionLock(key, tid)$\;
  }
}

\caption{MVCC-based transaction primitives.}
\label{alg:mvcc_txn_api}
\end{algorithm}


\subsubsection{Transaction Primitives}

In this section, we describes the transaction primitives implemented by wrapping up the storage APIs provided by the underlying UStore storage layer.
Alg~\ref{alg:mvcc_txn_api} provides details of the API design, and we summarize their functions as follows. 

{\bf Begin:} This primitive is used to start a new transaction. When initiating, a transaction gets a globally unique transaction
id and the snapshot descriptor from coordinator.

{\bf Read:} Transaction uses this primitive to fetch a record which it is allowed to read. If the record has an active version
which is not validated in the snapshot descriptor of this transaction, this transaction has to abort.

{\bf Write:} Transaction uses this primitive to update a record which it is allowed to write. Same as the \textbf{Read} primitive,
if the record has an active version which is not validated in the snapshot descriptor of this transaction,
this transaction has to abort.

{\bf Commit:} Transaction tries to commit in this primitive, where it tries to use the \textbf{Merge} API provided by storage layer to 
merge its updated version of records into the active version of the records. When this failed, this transaction needs to abort.

{\bf Abort:} During abort, all the updates made by this transaction are removed. 

\subsubsection{Life-cycle of Transaction Processing}

With the above transaction primitives, we are ready to depict the life-cycle of transaction processing. 
Referring to Figure~\ref{fig:MVCC}, each transaction is issued at a processing node and its processing needs to interact with the coordinator and the active version table. 
Initially per transaction, \funcBegin is called to prepare for the context of execution by constructing the snapshot. 
During the operational execution, \funcRead and \funcWrite are called for read and write operations respectively. 
Note that the read/write operations take effect in the transaction's private runtime space only. 
Upon transaction commit, data changes within the private space of transaction need to be materialized to the storage by calling \funcCommit at the end of the transaction execution.
If any kind of transaction abort occurs, \funcAbort is called accordingly.  


==> application_collaboration.tex <==
\subsection{Collaborative Analytics}

Another application that we present is collaborative analytics. In collaborative systems, two or more users (called
participants) work simultaneously on a shared computing system to achieve a common goal. In the case of collaborative
analytics, the common goal is to perform data science or business intelligence operations on the shared datasets.
Datasets can be large and git-like systems are not suitable for this application \cite{datahub}. In this section we show
a scenario for the collaborative analytics and show how \ustore can support building this application better than current systems.

\subsubsection{Scenario}

Electronic Medical Records (EMRs) are electronic storage systems that keep health information for individuals. These systems are common nowadays in hospitals and health care centers. Different users can work on this data as shown in Figure \ref{fig:collaborativeScenario}. The health information includes patient personal data, medical test results, diagnoses and prescriptions. This information is collected by different people (e.g. the reception desk, the nurse who made the test and the doctor who wrote the diagnosis). 

Furthermore, these records can be analyzed by data scientists. The data scientist can perform data cleaning and data analytics on the EMR. Data cleaning operations include, for instance, record deduplication and finding the code of a given diagnoses. Data analytics include classification, clustering and prediction \cite{gemini}. The quality of the results in the data analytics operation is enhanced if the data cleaning operations are performed first. The cleaning and the analytics operations are usually performed by different scientists that may work in different teams.

This scenario shows the need of a shared storage that support collaboration between all participants. While every one works on a small goal, such as recording test results or cleaning the dataset, the common goal is to provide better healthcare to the patients. Currently to achieve this common goal, the data must be transferred between different teams in an exchangeable format such as computer files or database dumps. Versioning is maintained manually using primitive and erroneous methods. Each participant or team may use a separate way to trace the provenance while working on the small goal but there is no global way to store provenance.

\begin{figure}
\centering
\includegraphics[width=0.25\textwidth]{collaborativeScenario.pdf}
\caption{An example for a collaborative scenario}
\label{fig:collaborativeScenario}
\end{figure}

\subsubsection{Awareness}

Collaborative awareness is the capacity to be aware of the current state of the collaboration \cite{collaborativeBook}.
If participants are aware of what their colleagues are doing on the shared goal, this could increase the productivity
and avoid conflicts. This awareness is implemented in computer collaborative systems by defining awareness policies and
developing notification systems that implement them. The awareness policy is application dependent and applications can
build their own policy with \ustore\ data structures and API.

In our scenario, the doctor may be notified when a new medical test result is written by the nurse to update his diagnoses. A data scientist who is going to run a classification algorithm on the dataset may wait if another colleague is currently running a cleaning operation on the same dataset. 

\subsubsection{Data Structures}
We base our solution on the mapping from Table view to Key-Value. In addition to the table, we introduce the \emph{Dataset} U-Object (See Figure \ref{fig:datasetUobject}). This object contains: (1) dataset meta data, such as title, owner and license. (2) List of pointers to files U-Objects and table U-Objects that belong to this dataset. The dataset API supports \emph{Add} and \emph{Remove} operations that adds files or tables to this dataset U-Object. The dataset meta data can be updated also using getter and setters in the API.

\begin{figure}
\centering
\includegraphics[width=0.20\textwidth]{datasetUobject.pdf}
\caption{The Dataset U-Object}
\label{fig:datasetUobject}
\end{figure} 

\subsubsection{Query Implementation}

We present here four sample queries adapted from \cite{decibel} and show how we can support them with \ustore. The
implementation can be done directly using the \ustore\ API or it can a use SQL engine if available. The usage of SQL
engine will allow us to implement the version-first or record-first representations as given in \cite{datahub}.
Nevertheless, we present here the direct implementation using \ustore\ API and keep the SQL engine implementation for the future work.

\begin{enumerate}

\item \emph{Single version scan}: a data scientist who runs a data analytics algorithm may need to read all tuples of
the table \emph{t} in the dataset \emph{d} for a given version \emph{v}. 

\item \emph{Multiple version positive diff}:  A doctor may want to know which patients were deleted in the new version
of the dataset. This query is executed by two single version scans as shown in the previous example. Then a diff
operation will be called to return the difference depending on the query conditions.

\item \emph{Multiple version join}: A nurse may want to collect some information about a patient (with name 'Sam')
represented in the table R from two versions v01 and v02. This query is executed also by two single version scans and
joining their results.

\item \emph{Find all head versions of a table}: A head version is the latest version in a branch. A data scientist may
want to perform his data cleaning tasks only on the latest version of a dataset \emph{d}. This query can be implemented
by a read operation from the Active Version Table that we present in \ref{label:mvcc:architecture}.

\end{enumerate}

\subsubsection{Novelty}

There are three main points that \ustore\ can offer which is novel. First, current dataset management systems such as
DataHub are built on relational databases, hence they suffer from scalability issues, while collaborative applications
that are built on \ustore\ can benefit from its advanced storage features. Second, \ustore\ will allow building
collaborative awareness which is not supported by current dataset sharing systems. Awareness feature aims to increase
productivity and acceptance of the system by making it more social through notifications. Implementing the awareness
feature on large scale is a challenge that can be met by the design of \ustore. Finally, current systems does not support table schema changes which are common operations in collaborate data cleaning and curation scenarios. 



==> background_git.tex <==
Git~\cite{git} is a widely used open-source distributed version control system (DVCS), which
provides speed and efficiency for maintaining source code in projects. It outperforms other VCS
(such as Subversion, CVS, Perforce), with unique features like cheap local branching, convenient
staging areas, and multiple workflows.

From the system perspective, immutability is one of the key characteristics that promises the
efficiency and effectiveness of Git. Immutability means that all content changes committed in Git
are permanently archived in version history. The Git backend can be viewed as an append-only
storage, with the abstract of a key-value store. For each commit, the changed content/files are
entirely archived in the backend storage as the value. After that, a key is deterministically
computed (e.g. SHA) from the value. As the result, given any commit key, Git is able to retrieve the
corresponding version from the backend. The immutability provided by the append-only key-value
storage gives Git three distinct advantages. First, it is straightforward and efficient to track the entire
version history. Second, it is easy to go back to any historical version, which is useful when it is
necessary to go back in time to a cleaner version. Third, it is easy to compare. Comparing two
branches is common in practice, and content-only comparison is inadequate, which can only tell
text-level differences, not version-based deep relations. Without the immutable history, it is even
impossible to handle automatic merging of two branches.

With immutable version history, Git is able to provide a higher level feature for version
controlling: mergeability. That is to merge two branches and resolve conflicts. However, conflict
resolving is always a challenge for collaborative project development. There are different
strategies used by Git to help resolve conflicts, i.e. fast-forward merge, three-way merge.
Fast-forward merge is used when a branch contains all the history of the other branch, along with
some more new commits at the end of the history. That means that at a previous point, two branches
are identical, and after that only one branch moves forward. In this case, it is straightforward to
apply all new commits to the other branch without involving any conflicts. If both branches evolve,
a 3-way merge algorithm is applied. The 3-way merge compares three versions of content, i.e., latest
versions in two branches and the version before two branches becoming diverse.  This strategy is
able to automatically resolve most conflicts without further effort. When the conflicts cannot be
resolved, the user will be notified to resolve them manually.  Overall, immutability and
mergeability make the management and evolvement of project more efficient. It let different
repositories update and communicate in a distributed and parallel manner.

In fact, immutability is becoming an inexorable trend for data-oriented
applications in recent years~\cite{immutability}.  Besides Git, it is also easy
to observe immutability in many other applications. Many massively parallel
computing systems, e.g., MapReduce and Dryad, are based on immutable inputs.
Most of these systems cut a single job into pieces, each of which takes
immutable inputs only and generates new immutable outputs, which are typically
stored on GFS or HDFS.  The immutable inputs and outputs makes them easy to
handle failures and restart a sub-task without complex coordination mechanism.
Spark is another state-of-the-art massive computing engine.  Its efficient and
effectiveness are highly based on the abstraction of RDDs, which are indeed
immutable datasets tracking the history of operations.

As mensioned, those high available file systems (e.g., GFS and HDFS) also
benefits a lot from immutability.  In these systems, each file is a bunch of
blocks (or chunks), which are immutable and typically created by single writer.
Such immutability allows files to be easily replicated across large clusters
for high availability, while avoids the propagation of updates.

Another successful example of immutability is from those LSM-like data
storages, such as levelDB and HBase.  In an LSM-tree, changes to the key-value
store are accomplished by writing new versions of the affected records.  All
new versions are appended to immutable log files, such that all historical
status of a record can be found easily.  Periodically, in order to remove
outdated content, immutable files are merged/compacted into smaller immutable
files containing only valid data.  Such appending and merging strategies
provides superior write-throughput for ingesting updates while simplifies the
failure recovery procedure.


==> challenges_hardware.tex <==

\subsection{How to utilize new hardware?}
Hardware solutions can boost the performance 
from the lowest underlying layers (i.e., transistors, circuits),
which usually does not introduce much overhead.
However, na\"{\i}ve adoption of hardware solutions does not guarantee superior performance
over software solutions.
  
  \textbf{Mismatch with traditional software/OS stack}.
  Newly-emerged hardware sometimes does not match with the traditional software/OS stack,
  which will cause unexpected behaviors or performance degradation.
  For example,
  although the byte addressability and durable writes of NVM render it perfect 
  for building an in-memory database,
  simply replacing DRAM or the disk with NVM to build an in-memory database 
  fails to take advantage of these features. This is
  because of the mismatch between block/page granularity of OS paging
  and the byte granularity of NVM,
  and the fact that the system is oblivious to the limited lifetime of NVM.
  The disparity in the write patterns between two partitions, 
  and the workload with high write skewness,
  can result in some NVM cells being written much more times
  and consequently worn out much earlier than others.
  This poses a stringent requirement for the wear-levelling algorithm.
  In addition, traditional file system requires
  \textit{read} or \textit{write} syscalls to access the file, 
  whose overhead can play a significant role in the total latency 
  when accessing NVM.
  
  \textbf{Scalability}.
  The scale of some new hardware cannot catch up with advances of other parts of the system,
  and some new hardware cannot easily scale up/out without significant performance degradation.
  For example, it is not uncommon that 
  a multicore machine has more than 100 cores and hundreds or thousands gigabytes of memory, 
  but HTM can only scale to a limited number of CPU cores {\cite{leis2014exploiting}},
  and Xeon Phi coprocessor can only support up to 16 GB memory.
  Doubts have also been raised on the scalability of 
  some of the RDMA solutions~\cite{ethernetroce}.  
  RDMA memory consumption also poses a big challenge on large cluster
  due to the flexibility of communication model and user-dependent message passing implementation,
  losing the advantages that can be derived from mature network stack mechanism and memory management by OS.

  Another scalability issue is that the current hardware support 
  for virtual memory does not scale to terabytes (and beyond) of physical memory. The use of small page sizes and fine
  protection boundaries will require significant space overhead in the corresponding page
  tables. The na\"{\i}ve solution of enlarging page sizes is only a stop-gap measure as it
  will eventually lead to large page protection boundaries, fragmentation, and 
  inefficient use of memory.

  \textbf{Generality/Compatibility}.
  Hardware solutions are usually architecture specific, 
  and not general enough to satisfy the different requirements
  from a variety of applications.
  For example, RDMA cannot easily communicate with the traditional
  Ethernet network directly.
  In addition, not all database transaction semantics can be expressed using HTM, 
  since there are some other factors restricting its usage,
  e.g., limited HTM transaction size that is restricted by L1 cache,
  unexpected transaction abort due to cache pollution problems.
  Moreover, data alignment requirement for SIMD makes SIMD-based implementation
  architecture specific.
    
  \textbf{Extra overhead}.
  In order to utilize some hardware, there are extra preparation work to do,
  which may offset the performance gain from the hardware.
  For example, in order to use SIMD instructions,
  we need to gather data into SIMD registers and 
  scatter it to the correct destination locations,
  which is tricky and can be inefficient.
  RDMA only allows a pre-registered memory region
  to be the transmission source/destination,
  which also cannot be released/modified until the transmission is completed.
  
  \textbf{Bottleneck shift}.
  Even though the use of new hardware may tackle one bottleneck, 
  the contribution to the system's overall performance may be restricted. 
  In some cases, it only results in a bottleneck shift.
  For instance, the adoption of RDMA usually moves the bottleneck
  from network I/O to CPU,
  as with a fast networking,
  CPU is usually busy with data preparation and notification checking~\cite{kalia2014rdma,memepiccite}.
  And even though HTM can reduce the overhead caused by concurrency control to some extent,
  some components such as durability and communication still restrict the overall performance.

==> challenges_security.tex <==
\subsection{Challenges in Security}
{\bf Threat model.} Security-sensitive applications must now consider a strong threat model to account for
powerful, highly motivate adversaries, as well as the complexity of software stack, and the availability of
side-channels~\cite{side_channel_image}. One example is to assume that the adversary has complete
access to the software (or hardware) stack, either via malicious use of admin privilege (insider) or via
exploiting of software vulnerabilities. A strong threat model demands strong (and often complex) security
mechanisms.    

{\bf Privacy preserving computation on data.} When data is outsourced to an untrusted party, data privacy is
often ensured via encryption. However, existing encryption schemes are either too costly, too limited in
functionality or too weak to be practical. By leveraging trusted computing primitives (hardware or software),
it is possible to bring down the performance overheads while maintaining semantic security. While trusted
computing can protect data within the unit of computation, there are still other channels of data leakage via
memory and I/O access patterns, especially when the computation is
distributed~\cite{m2r,ohrimenko15}. Another challenge with this approach is how to minimize
the trusted computing base (TCB), as a large TCB increases the
attack surface. 

{\bf Data provenance.} Most existing works consider protecting integrity of data provenance by ensuring fork
consistency. Confidentiality of the data history is equally important in collaborative environments, but it
has largely been ignored. SPORC~\cite{sporc} is one of the exceptions, but its scope is limited to document
editing. Decentralized systems like Bitcoin or Etherum also make the ledger public, giving rise to  
de-anonymizing attacks~\cite{deanonymize_bitcoin}. Achieving both integrity and confidentiality for data
provenance in multi-user, untrusted environment remains a challenge.       

{\bf Performance overhead.} Providing data confidentiality guarantees always leads to performance overhead. The latter
is attributed to the additional storage required for ciphertexts, and the additional CPU cycles spent in
processing encrypted data. When trusted computing primitives are used, there is an extra cost in setting up,
tearing down and switching into the trusted execution environment. Achieving practical performance for systems
with confidentiality requirements remains a challenge. While systems that focus on integrity, such as Bitcoin, can
tolerate certain overhead with respect to data update, there is an increasing demands for faster response
time at the cost of security~\cite{ethereum}.  



==> challenges_sharing.tex <==
\subsection{Challenges in Sharing and Collaboration}
{\bf Throughput and latency.} Most data sharing and collaborative services are now being offered by cloud providers. The
tremendous amount of data being shared demands high throughput from the system. Furthermore, many applications such as
photo sharing and real-time collaboration are latency sensitive. Meeting both throughput and latency requirements at
scale is still a challenge. For example, Git is known to perform badly with large files~\cite{git_scalability}. The need
for performance at scale is also driven by collaborative big-data analytics~\cite{adam_sigmod15}. Existing works propose
  new data models~\cite{datahub} or fundamental changes to the storage~\cite{fds,haystack} and networking
  stack~\cite{never_than_late}, but they target limited sets of workloads, and may not work consistently well  across
  different sharing and collaborative models.   

{\bf Conflicts.} Another challenge in collaborative systems is how to deal with update conflicts. For many systems where
updates are infrequent or where application semantics are not specified, conflict resolutions are left to the users
(Git, Dropbox, for example). However, user interference is undesirable for real-time systems wherein changes are
propagated in real time. GoogleDocs, for instance, uses an efficient, lock-free technique called operational
transformation (OT)~\cite{ot} to automatically resolve conflict.  An alternative to OT is to let user defines
application-specific merge functions which are automatically applied to update conflicts when detected~\cite{bayou}.  

{\bf Access control.} Providing access control in sharing and collaborative applications presents two main challenges.
First, the access control model must be expressive enough to support fine-grained policies based on the
data content, in addition to the coarse-grained, role-based model~\cite{blind_enforcer}. It is also desirable for the
model to be formally verified and proved for its safety property. Second, without a trusted party, the enforcement of
access control must be done via cryptographic techniques which may restrict the policy's expressiveness and may incur
large overhead~\cite{streamforce}. 




==> challenges_summary.tex <==
\subsection{Summary}
\begin{table*}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|l|p{8cm}|}
\hline
{\bf Property} & {\bf Challenges} \\ \hline
\multirow{2}{*}{\em Immutability} & 1. Storage, data representation for immutable objects \\
& 2. Thoughput, latency in retrieving, updating.  \\ \hline
\multirow{3}{*}{\em Versioning} & 3. Frequency of versioning \\ 
& 4. What to version: granuality of data \\ 
& 5. How to save storage: pruning, compression \\ \hline 
\multirow{3}{*}{\em Sharing \& Collaboration} & 6. Throuhput and latency: how much, how fast \\
& 7. Conflict management: how to detect, how to resolve conflict \\
& 8. Access control: who to share, what to share \\ \hline
\multirow{3}{*}{\em Security} & 9. Data privacy and integrity: what to protect, how to protect \\
& 10. Privacy-preserving computation: computation over encrypted domains \\
& 11. Performance: low overhead \\ \hline
\multirow{2}{*}{\em Utilizing new hardware} & 12. Mismatch with traditional OS, application software stack: ease of
integration, of programming \\
& 13. Incommensurate scaling: different hardware scale differently, shifting in bottleneck \\ \hline
\end{tabular}
}
\caption{Summary of research challenges}
\label{tab:challenges}
\end{table*}


==> challenges_versioning.tex <==
\subsection{Design Issues of Data Versioning}

When designing a data versioning system, two core design issues are mainly concerned: how to keep track of individual versions (i.e., the completeness issue), and how to store each version in a storage-efficient way (i.e., the storage issue). 

\textbf{Completeness.} 
The completeness of data versioning decides the amount of versioning information the version repository retains. 
The more complete is the information, the less possible is the data loss and the stronger support it has for history study. 
The completeness is specified in terms of versioning frequency, versioning scope, and pruning strategy.

First, \textit{versioning frequency} refers to the issue of when to save a version. 
One extreme is \textit{comprehensive versioning} where every update of data object is saved. 
With comprehensive versioning, it is possible to recover from any kind of data loss and to provide strong support for history study. 
Another extreme is mirror data system where only one recent version is kept, it is mainly used to protect the data system from hardware failure. 
Other schemes selectively save versions. 
Versions can be specified in a \textit{regular} manner, i.e., at fixed time interval such as weekly, daily or hourly versioning. 
It can be flexibly controlled \textit{on demand} by user as in Git~\cite{git}.
More advanced schemes let data versioning system \textit{automatically} decide when to save a version based on statistics and heuristics. 
Obviously, automatic versioning is attractive but its design towards comprehensive automation turns out to be challenging. 

Second, \textit{versioning scope} means the portion of a data system which is subject to versioning. 
It can be the whole data system or partial data system or flexibly controlled by user. 
General cases for partial data systems are one or more logical partition or databases. 
For example, system administrator may specify the \texttt{/home} partition to be backup while excluding the \texttt{/tmp} partition. 
Using Git-like systems, user has finely control over which files to be versioned.
However, for complicated applications, defining proper versioning scopes may not be straightforward. 
For example, in a column-store-based storage system, enforcing the versioning in a row-based scope would contradict the storage structure which is column-based, whereas enforcing the versioning in a column-based scope would lead to high redundancy of data among versions. 
In general, defining comprehensive abstractions of versioning scope as well as providing the corresponding implementation support are challenging. 

Third, \textit{pruning strategy} decides when to discard a version in the version repository. 
One extreme is to never prune, as in Git~\cite{git}. 
Another strategy keeps a period of time for each version which we call \textit{prune window}. 
The window length can be simply predefined by system administrator, and meanwhile limited by hardware resource consumption or by performance requirement. 
For example, a data system may dedicate 20\% of its storage capacity for data versioning. 
These factors are correlated. 
Too much hardware resource consumption usually will lead to performance degradation of accessing current objects or old versions. 
When system administrators define the prune window length, resource consumption and performance degradation are two important criterion. 
More flexible strategy assumes different data object have different requirement for window length. 
Even for the same object, some version may be more important than other versions and need to be kept for a longer period. 
Therefore, \textit{selective pruning} plays a critical role in managing the resource usage of the data versioning system.
However, the decision scheme of selective pruning requires multi-dimension monitoring and adaptive tuning to achieve its optimal or near-optimal performance. 
Designing the building blocks of selective pruning for various data versioning applications is challenging. 

\textbf{Storage.}
The hardware resources consumed by data versioning include storage capacity, storage bandwidth, network bandwidth and CPU power. 
Multiple versions of a data object need extra space to store. 
They also need storage bandwidth to be transferred to the media. 
If version repository is in a remote site, the transfer need to consume network bandwidth. 
Extra CPU time is needed to save, represent and extract versions. 
Versioning system can exchange CPU with other types of resources. 
By using more CPU time on differencing and compression algorithm, storage capacity, storage bandwidth and network bandwidth can be saved. 
This corresponds to the trade-off between CPU resources and storage/bandwidth resources. 

How much resource a data versioning system consumes depends on three factors: the workload, the versioning completeness, and the organization of version repository. 
The workload refers to the update percentage of data access operations. 
Versioning completeness is described as aforementioned. 
The organization of version repository refers to the location and layout of version repository. 
Out of the three factors, the workload is decided by the application, the completeness is mostly a design decision, and the organization of version repository remains an open research area.
It is a challenging task to build up an organization framework of version repository that is not only applicable to diverse layouts of version repository, but also compatible with the design of the completeness of data versioning.  


==> overview.tex <==
% explaining the stack 
\subsection{Overview}
Figure~\ref{fig:stack} shows multiple layers of UStore stack. At the bottom, the physical layer is responsible
for storing, distributing and replicating data over many servers. We consider settings in which servers belong
to a number of independent administrative domains, i.e. they are mutually distrustful. At the next layer,
i.e. data representation layer, lies the UStore's core data structure which bears some similarity to Git's.
In particular, it implements immutability with support for branching and merging. However, UStore
differentiates from Git in the structure and operational semantics of each data value. The distinction to Git
becomes more apparent at the next two layers. The APIs layer exposes access operations which are specific to a
version of data.The view layer enhances the immutability semantics of the data structure with fine-grained
access control, security and consistency model.   Finally, applications exploiting UStore's rich semantics can
be built directly on the APIs and the views from the lower layers. Transactional systems, collaborative
systems are two of many examples that directly benefit from using UStore. 

The Git-like data structure embedded at the second layer makes up the narrow waist of the design. In other
words, UStore allows for a single representation and unchanged semantics of this data structure, but different
physical, view and application layers are possible. We remark that this narrow-waist design is inspired by the
success of the TCP/IP networking stack. By fixing the representation, UStore can easily accommodate
innovations at the physical layer and changes in application requirements. 

We now discuss how the layered design in Figure~\ref{fig:stack} helps achieving the four goals laid out
earlier. First, UStore semantics (G1) are realized by the data representation and view layer. Second, UStore's
flexibility (G2) are achieved by exposing parameters at the physical layers for specifying constraints on
resources, on distribution and replication strategies.  Furthermore, the APIs return all relevant versions,
making it general for many applications. In addition, UStore does not enforce a specific consistency model,
i.e. applications can overwrite the consistency view to implement their own models. Third, UStore's efficiency
and scalability (G3) comes from the careful use of the available hardware at the physical layer. Finally, the
ease of development (G4) follows from the APIs which hide complexity of managing data in distributed settings.
Application developers can also benefit directly from the set of pre-built views to implement sharing and
consistent views of data.  


